Convex Program Duality, Fisher Markets, and Nash Social Welfare

We study Fisher markets and the problem of maximizing the Nash social welfare (NSW), and show several closely related new results. In particular, we obtain: -- A new integer program for the NSW maximization problem whose fractional relaxation has a bounded integrality gap. In contrast, the natural integer program has an unbounded integrality gap. -- An improved, and tight, factor 2 analysis of the algorithm of [7]; in turn showing that the integrality gap of the above relaxation is at most 2. The approximation factor shown by [7] was $2e^{1/e} \approx 2.89$. -- A lower bound of $e^{1/e}\approx 1.44$ on the integrality gap of this relaxation. -- New convex programs for natural generalizations of linear Fisher markets and proofs that these markets admit rational equilibria. These results were obtained by establishing connections between previously known disparate results, and they help uncover their mathematical underpinnings. We show a formal connection between the convex programs of Eisenberg and Gale and that of Shmyrev, namely that their duals are equivalent up to a change of variables. Both programs capture equilibria of linear Fisher markets. By adding suitable constraints to Shmyrev's program, we obtain a convex program that captures equilibria of the spending-restricted market model defined by [7] in the context of the NSW maximization problem. Further, adding certain integral constraints to this program we get the integer program for the NSW mentioned above. The basic tool we use is convex programming duality. In the special case of convex programs with linear constraints (but convex objectives), we show a particularly simple way of obtaining dual programs, putting it almost at par with linear program duality. This simple way of finding duals has been used subsequently for many other applications.

==> ExistanceAndUniqueness.tex <==
\section{Existence and Uniqueness}

In this section, we study the existence and the uniqueness of equilibria for the market models. 
For model $\mathcal{M}_1$, we show a necessary and sufficient condition for the existence of an equilibrium. The condition works for both cases of linear utility and spending constraint utility. On the uniqueness side, we show the spending vector, $q=(q_1,\ldots,q_m)$ where $q_j$ is the money spent on good $j$, is unique. 
For model $\mathcal{M}_2$, we show that an equilibrium always exists for all utility functions we mentioned in the previous section. On the uniqueness side, the utility vector is unique.

Despite the fact that in Fisher model we have the uniqueness of price equilibrium, it is easy to see that it is not true in our generalizations.
For model $\CM_1$, consider a market with only one buyer with utility function $u(x)=x_1$ and one seller. Let $m_1=1$ and $\SB=1$. It is easy to see every price in bigger than 1 is an equilibrium price.  
For model $\CM_2$, again consider a market with only one buyer with utility function $u(x)=x_1$ and one seller. Let $\UB_1=1$ and $m_1=2$. It is easy to see every price in interval $[1,2]$ is an equilibrium price.  




\subsection{Market $\CM_1$: Sellers have earning limits} 
\begin{lemma} \label{earning_existence}
 In model $\mathcal{M}_1$ under linear and spending constraint utility functions, an equilibrium price exists if and only if $\sum_j \SB_j \geq \sum_i m_i$. 
\end{lemma}
\begin{proof} An equilibrium price exists if and only if the feasible region of the convex program is not empty. We first prove that for the case of linear utility function, the program is feasible if and only if $\sum_j \SB_j \geq \sum_i m_i$. If $\sum_j \SB_j < \sum_i m_i$ then the feasible region is empty because the set of constraints \ref{con1.1}, \ref{con1.2} and \ref{con1.3} can not be satisfied together. If $\sum_j \SB_j \geq \sum_i m_i$ then $y_{ij} = \frac{m_i \SB_j}{ \sum_j \SB_j}$ gives a feasible solution because $\sum_i y_{ij} = \SB_j \frac{\sum_i m_{i}}{\sum_j \SB_j} \leq \SB_j$ and $\sum_j y_{ij} = m_i \frac{\sum_j \SB_{j}}{\sum_j \SB_j} = m_i$. 

Similarly, we can prove that  for the case of spending constraint utility, the program is feasible if and only if $\sum_j \SB_j \geq \sum_i m_i$. If $\sum_j \SB_j < \sum_i m_i$ then the feasible region is empty because the set of constraints \ref{con5.1}, \ref{con5.2} and \ref{con5.3} can not be satisfied together. Using a similar argument as in the previous part, we can show that if the amount of money that $i$ spends on $j$ is $m_i \SB_j /  \sum_j \SB_j$ then constraints \ref{con5.1}, \ref{con5.2} and \ref{con5.3} are all satisfied. We only need to guarantee that contraint \ref{con5.4} is satisfied as well. This can be done by choosing appropriate $y_{ij}^l$'s such that 
$ \sum_l y_{ij}^l =  \frac{ m_i \SB_j}{\sum_j \SB_j} \qquad \text{and} \qquad y_{ij}^l  \leq B_{ij}^l. $
\end{proof}

\begin{lemma}
In model $\mathcal{M}_1$ under linear and spending constraint utility functions, the spending vector $q$ is unique.
\end{lemma}

\begin{proof}
Consider two distinct price equilibriums $p$ and $p'$, their corresponding spending vectors $q$ and $q'$ and their corresponding demand vectors $x$ and $x'$.
Note that $p_j \geq p'_j \Rightarrow q_j\geq q'_j$ because $q_j=x_j p_j= \min (1,\frac{\SB_j}{p_j})p_j\geq \min (1,\frac{\SB_j}{p'_j})p'_j=q'_j$. 
Consider price vector $r=(r_1,\ldots,r_m)$ where $\forall k,$ $r_k= \max (p_k,p'_k)$, its corresponding spending vector $q^r$ and its corresponding demand vectors $x^r$.
Note that by changing prices from $p$ to $r$ we may only increasing the prices. Therefore, it is easy to see under linear or spending constraint utility functions the demand of good $j$ going from prices $p$ to $r$ would not decrease if $p'_j<p_j=r_j$. 
%
%Note that for both linear and spending constraint utilities , the demand of good $j$, $x_j$, will not decrease with changing prices from $p$ to $r$ if $r_j=p_j$ because 
Therefore, 
we have $ q^r_j=x^r_j r_j=x^r_j p_j\geq x_j p_j=q_j\geq q'_j$. We can do the same for all $j$ and show $\forall j,$ $q^r_j=max(q_j,q'_j)$.
For the sake of a contradiction suppose $\exists j$, $q_j>q'_j$ then using the later it is easy to show $\sum_j q^r_j > \sum_j q_j = \sum_j q'_j=\sum_i m_i$ which is contradiction because the money spent on goods cannot be more than the total budget. Therefore, $\forall j$ , $q_j=q'_j$ and the lemma follows.
\end{proof}

\subsection{Market $\CM_2$: Buyers have utility limits}

\begin{lemma} \label{utility_existence}
In model $\CM_2$ under linear, Leontief and CES utility functions, an equilibrium price always exists. 
\end{lemma}
\begin{proof} An equilibrium price exists if and only if the feasible region of the convex program is not empty. In \ref{cp1}, \ref{cp2} and \ref{cp3}, $x_{ij} = 0$ for all $i \in B,j \in A$ is a feasible solution. Therefore, the feasible region is not empty and an equilibrium exists.
\end{proof}
\begin{lemma}
In model $\CM_2$ under linear, Leontief and CES utility functions, the utilities of an equilibrium are unique.
\end{lemma}
%\vspace{-3}
\begin{proof}
In section \ref{utility_bound_section}, we showed every equilibrium correspond to an solution of a convex program with an objective function of the form $\sum_{i} m_i \log u_i$.
It is easy to see that the objective function is strictly concave.
Therefore, there is a unique vector $u$ that maximizes the objective function and the lemma follows.
\end{proof}

==> macros.tex <==
 \newenvironment{proof}{\noindent {\bf Proof:}}{$\Box$ \medskip}
% \newenvironment{proofoffact}{\noindent {\sc Proof of Fact:}}{$\Box$ \medskip}
% \newenvironment{proofofclaim}{\noindent {\sc Proof of Claim:}}{$\Box$ \medskip}
% \newenvironment{proofoflemma}{\noindent {\sc Proof of Lemma:}}{$\Box$ \medskip}

%%Version Feb 3 2001; last edited by SA
% Feb 13, 2001: LT adds following macros:
%  \logred, \conl, \genclass, \cogenclass, \size,
%  \floor, \ceil, \comp, \ffigure, \ffigureh
%  \iff, \implies, \sigmatwo, \sigmathree, \pitwo,
%  \scand, \scor, \scnot, \scyes
%Feb20 SA added \sig and \pip for boldface polynomial hierarchy
%% Macros for complexity theory notation
%% Complexity classes
\renewcommand\P{\mbox{\bf P}\xspace}
\newcommand\NP{\mbox{\bf NP}\xspace}
\newcommand\cnp{\mbox{\bf coNP}\xspace}
\newcommand\sigmatwo{\mbox{\bf $\Sigma_2$}\xspace}
\newcommand\sigmathree{\mbox{\bf $\Sigma_3$}\xspace}
\newcommand\pitwo{\mbox{\bf $\Pi_2$}\xspace}
\newcommand\rp{\mbox{\bf RP}\xspace}
\newcommand\zpp{\mbox{\bf ZPP}\xspace}
\newcommand\bpp{\mbox{\bf BPP}\xspace}
\newcommand\ph{\mbox{\bf PH}\xspace}
\newcommand\pspace{\mbox{\bf PSPACE}\xspace}
\newcommand\npspace{\mbox{\bf NPSPACE}\xspace}
\newcommand\dl{\mbox{\bf L}\xspace}

\newcommand\conl{\mbox{\bf coNL}\xspace}
\newcommand\sharpp{\mbox{\#{\bf P}}\xspace}
\newcommand\parityp{\mbox{$\oplus$ {\bf P}}\xspace}
\newcommand\ip{\mbox{\bf IP}\xspace}
\newcommand\pcp{\mbox{\bf PCP}}
\newcommand\dtime{\mbox{\bf DTIME}}
\newcommand\ntime{\mbox{\bf NTIME}}
\newcommand\dspace{\mbox{\bf SPACE}\xspace}
\newcommand\nspace{\mbox{\bf NSPACE}\xspace}
\newcommand\cnspace{\mbox{\bf coNSPACE}\xspace}
\newcommand\exptime{\mbox{\bf EXPTIME}\xspace}
\newcommand\nexptime{\mbox{\bf NEXPTIME}\xspace}
\newcommand\genclass{\mbox{$\cal C$}\xspace}
\newcommand\cogenclass{\mbox{\bf co$\cal C$}\xspace}
\newcommand\size{\mbox{\bf SIZE}\xspace}
\newcommand\sig{\mathbf \Sigma}
\newcommand\pip{\mathbf \Pi}

%%Computational problems

\newcommand\sat{\mbox{SAT}\xspace}
\newcommand\tsat{\mbox{3SAT}\xspace}
\newcommand\maxtsat{\mbox{MAX3SAT}\xspace}
\newcommand\tqbf{\mbox{TQBF}\xspace}


%% Notation for integers, natural numbers, reals, fractions, sets, cardinalities
%%and so on

\newcommand\bz{\mbox{\bf Z}}
\newcommand\nat{\mbox{\bf N}}
\newcommand\rea{\mbox{\bf R}}
\newcommand\B{\{0,1\}}      % boolean alphabet  use in math mode
\newcommand\Bs{\{0,1\}^*}   % B star            use in math mode
\newcommand\true{\mbox{\sc True}}
\newcommand\false{\mbox{\sc False}}
\DeclareRobustCommand{\fracp}[2]{{#1 \overwithdelims()#2}}
\DeclareRobustCommand{\fracb}[2]{{#1 \overwithdelims[]#2}}
\newcommand{\marginlabel}[1]%
{\mbox{}\marginpar{\it{\raggedleft\hspace{0pt}#1}}}
\newcommand\card[1]{\left| #1 \right|} %cardinality of set S; usage \card{S}
\newcommand\set[1]{\left\{#1\right\}} %usage \set{1,2,3,,}
%\newcommand\poly{\mbox{poly}}  %usage \poly(n)
\newcommand{\floor}[1]{\lfloor\, $#1$\,\rfloor}
\newcommand{\ceil}[1]{\lceil\, $#1$\,\rceil}
\newcommand{\comp}[1]{\overline{#1}}


%% Various things to write in small caps

\def\scand{\mbox{\sc and}}
\def\scor{\mbox{\sc or}}
\def\scnot{\mbox{\sc not}}
\def\scyes{\mbox{\sc yes}}


%% short-hands for relational simbols

%\newcommand\to{\rightarrow}
\newcommand{\from}{:}
\newcommand\xor{\oplus}
\newcommand\bigxor{\bigoplus}
\newcommand{\logred}{\leq_{\log}}
\def\iff{\Leftrightarrow}
\def\implies{\Rightarrow}


%% probability stuff
\newcommand\prob{\mbox{\bf Pr}}
\newcommand\E{\mbox{\bf E}}
\newcommand\var{\mbox{\bf Var}}



%% macros to write pseudo-code

\newlength{\pgmtab}  %  \pgmtab is the width of each tab in the
\setlength{\pgmtab}{1em}  %  program environment
 \newenvironment{program}{\renewcommand{\baselinestretch}{1}%
\begin{tabbing}\hspace{0em}\=\hspace{0em}\=%
\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=%
\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=%
\+\+\kill}{\end{tabbing}\renewcommand{\baselinestretch}{\intl}}
% \newcommand {\BEGIN}{{\bf begin\ }}
% \newcommand {\ELSE}{{\bf else\ }}
% \newcommand {\IF}{{\bf if\ }}
% \newcommand {\FOR}{{\bf for\ }}
% \newcommand {\TO}{{\bf to\ }}
% \newcommand {\DO}{{\bf do\ }}
% \newcommand {\WHILE}{{\bf while\ }}
% \newcommand {\ACCEPT}{{\bf accept}}
% \newcommand {\REJECT}{\mbox{\bf reject}}
% \newcommand {\THEN}{\mbox{\bf then\ }}
% \newcommand {\END}{{\bf end}}
% \newcommand {\RETURN}{\mbox{\bf return\ }}
% \newcommand {\HALT}{\mbox{\bf halt}}
% \newcommand {\REPEAT}{\mbox{\bf repeat\ }}
% \newcommand {\UNTIL}{\mbox{\bf until\ }}
% \newcommand {\TRUE}{\mbox{\bf true\ }}
% \newcommand {\FALSE}{\mbox{\bf false\ }}
% \newcommand {\FORALL}{\mbox{\bf for all\ }}
% \newcommand {\DOWNTO}{\mbox{\bf down to\ }}

%% %formatting commands
%% \newcounter{lecnum}
%% \newcommand{\lecture}[3]{%
%% \pagestyle{myheadings}%
%% \thispagestyle{plain}%
%% \newpage %
%% \setcounter{lecnum}{#1}%
%% \setcounter{page}{1}%
%% %\rule{\linewidth}{1mm}
%% \begin{center}
%% \shadowbox{\parbox{4.3in}{{\small {\bf {\sc Georgia Tech  Fall'04
%%  \\ \hfill CS 8002 : PCPs and Hardness of Approximation}}}

%% \medskip

%% \begin{center}
%% {\large Lecture #1: #2}
%% \end{center}

%% \medskip

%% Lecturer: {\em Subhash Khot} \hfill Scribe:{\em #3}
%% \vspace{2pt}}}
%% \vspace{6pt}\end{center}}

%% %%%%%%%%    SPRING'01
%% \newcommand{\coursenum}{CS278}
%% \newcommand{\coursename}{Computational Complexity}
%% \newcommand{\courseprof}{Professor Luca Trevisan}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commands to include figures


%% PSfigure

\newcommand{\PSfigure}[3]{\begin{figure}[t]
  \centerline{\vbox to #2 {\vfil \psfig{figure=#1.eps,height=#2} }}
  \caption{#3}\label{#1}
  \end{figure}}

\newcommand{\twoPSfigures}[5]{\begin{figure*}[t]
  \centerline{%
    \hfil
    \begin{tabular}{c}
        \vbox to #3 {\vfil\psfig{figure=#1.eps,height=#3}} \\ (a)
    \end{tabular}
    \hfil\hfil\hfil
    \begin{tabular}{c}
        \vbox to #3 {\vfil\psfig{figure=#2.eps,height=#3}} \\ (b)
    \end{tabular}
    \hfil}
  \caption{#4}
  \label{#5}
%  \sublabel{#1}{(a)}
%  \sublabel{#2}{(b)}
  \end{figure*}}


\newcounter{fignum}

% fig
%command to insert figure. usage \fig{name}{h}{caption}
%where name.eps is the postscript file and h is the height in inches
%The figure is can be referred to using \ref{name}
\newcommand{\fig}[3]{%
\begin{minipage}{\textwidth}
\centering\epsfig{file=#1.eps,height=#2}
\caption{#3} \label{#1}
\end{minipage}
}%


% ffigure
% Usage: \ffigure{name of file}{height}{caption}{label}
\newcommand{\ffigure}[4]{
\begin{figure}
\caption{#3}
\label{#4}
\centerline{\vbox to #2 {\hfil \psfig{figure=#1.eps,height=#2} }}
\end{figure}
}

% ffigureh
% Usage: \ffigureh{name of file}{height}{caption}{label}
\newcommand{\ffigureh}[4]{
\begin{figure}[!h]
\caption{{\small {\sc #3}}}
\label{#4}
\centerline{\vbox to #2 {\vfil \psfig{figure=#1.eps,height=#2} }}
\end{figure}
}

\newcommand{\pdffigureh}[4]{\begin{figure}[!h]
  \centerline{\vbox to #2 {\vfil \pdffig{figure=#1.eps,height=#2} }}
  \caption{{\small {\sc #3}}}\label{#4}
  \end{figure}}

%beautifications
\def\bsq{\begin{flushright}$\blacksquare$\end{flushright}}
\def\ni{\noindent}


%mystuff


\newcommand{\opt}{\mbox{\rm OPT}}
\newcommand{\alg}{\mbox{\rm ALG}}
\renewcommand{\deg}{\mbox{\rm deg}}
\newcommand{\outdeg}{\mbox{\rm outdeg}}
\newcommand{\ra}{\rightarrow}
\newcommand{\R}{\mbox{\rm\bf R}}
\newcommand{\Rplus}{\R_+}
\newcommand{\minimize}{\mbox{\rm minimize }}
\newcommand{\maximize}{\mbox{\rm maximize }}
\newcommand{\parent}{\mbox{\rm parent }}
\newcommand{\st}{\mbox{\rm subject to }}
\newcommand{\C}{\mbox{${\cal C}$}}
\newcommand{\F}{\mbox{${\cal F}$}}
\newcommand{\li}{\mbox{${\lambda_i}$}}
\renewcommand{\O}{\mbox{${\cal O}$}}
%\renewcommand{\aa}{\mbox{$\alpha$}}
\newcommand{\ah}{\mbox{$\aa_{INC}$}}
%\renewcommand{\bb}{\mbox{\boldmath $\beta$}}
%\newcommand{\bh}{\mbox{$\bb_{INC}$}}
\renewcommand{\tt}{\mbox{\boldmath $t$}}
\newcommand{\rr}{\mbox{\boldmath $r$}}
\newcommand{\at}{\mbox{$\tt_{INC}$}}
\newcommand{\ar}{\mbox{$\rr_{INC}$}}
\newcommand{\aq}{\mbox{$\qq_{INC}$}}
\newcommand{\x}{\mbox{\boldmath $x$}}
\newcommand{\y}{\mbox{\boldmath $y$}}
\newcommand{\z}{\mbox{\boldmath $z$}}
\newcommand{\e}{\mbox{\boldmath $e$}}
\def\p{\mbox{\boldmath $p$}}
\def\q{\mbox{\boldmath $q$}}
%\def\q{{\boldmath q \unboldmath}}
\def\X{{\mbox{\boldmath $X$}}}
\def\x{\mbox{\boldmath $x$}}
\def\e{\mbox{\boldmath $e$}}
\def\U{\mbox{\boldmath $U$}}
\def\a{\mbox{\boldmath $s$}}
\def\s{\mbox{\boldmath $s$}}
\def\m{\mbox{\boldmath $m$}}
\def\b{{\bf b}}
\def\Int{\mbox{\rm Int}}
\def\eps{\epsilon}
\def\uij{u_{ij}}
\def\uijl{u_{ij}^l}
\def\Bijl{B_{ij}^l}
\def\lijk{l_{ij}^k}
\def\g{\mbox{\boldmath $g$}}
\def\f{\mbox{\boldmath $f$}}
\newcommand{\lone}[1]{\ensuremath{|#1|}}
\newcommand{\Real}{\mbox{\rm\bf R}}
\newcommand{\A}{\mbox{\boldmath $\alpha$}}
%\newcommand{\B}{\mbox{\boldmath $\beta$}}
\newcommand{\ga}{\mbox{\boldmath $\gamma$}}
\newcommand{\ltwo}[1]{\|#1\|}
\newcommand{\Cs}{\mbox{{\cal C}}}
%\newcommand{\L}{\mbox{${\cal L}$}}
\newcommand{\Z}{\mbox{\rm\bf Z}}
\newcommand{\Zplus}{\Z^+}
\newcommand{\CA}{\mbox{${\cal A}$}}
\renewcommand{\span}{\mbox{\rm span}}


\newcommand{\pp}{\mbox{\boldmath $p$}}
\newcommand{\mm}{\mbox{\boldmath $m$}}
\renewcommand{\aa}{\mbox{\boldmath $a$}}
\renewcommand{\ss}{\mbox{\boldmath $s$}}
\newcommand{\bp}{\mbox{$\pp_{DEC}$}}
\newcommand{\ap}{\mbox{$\pp_{INC}$}}
\newcommand{\bq}{\mbox{$\qq_{DEC}$}}
\newcommand{\br}{\mbox{$\rr_{DEC}$}}
%\newcommand{\implies}{\mbox{${\Rightarrow}$}}
\newcommand{\eat}[1]{}

\newcommand{\maxi}{{\hbox{\rm maximize}}}
\newcommand{\mini}{{\hbox{\rm minimize}}}
\newcommand{\subjto}{{\hbox{\rm subject to}}}
%\newcommand{\text}[1]{\hbox{\rm #1}}

\def\d{\displaystyle}

\newcommand{\assign}{\leftarrow}


\renewcommand{\u}{\mbox{\boldmath $u$}}
\renewcommand{\v}{\mbox{\boldmath $u$}}
\def\c{{\bf c}}
\renewcommand{\t}{\mbox{\boldmath $t$}}
%\newcommand{\m}{\mbox{\boldmath $m$}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Pu}{\mathcal{P}_u}
\newcommand{\Pf}{\mathcal{P}_f}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\D}{\mathcal{D}}


\newcommand{\ipj}{\ensuremath{I_{j,j+1}}}
\newcommand{\ipl}{\ensuremath{I_{l,l+1}}}

\newcommand{\aij}{ a_{ij}}
\newcommand{\cij}{ c_{ij}}
\newcommand{\akj}{ a_{kj}}
%\newcommand{\uij}{ u_{ij}}
\newcommand{\xij}{ x_{ij}}
\newcommand{\aijp}{ a_{kj}}
\newcommand{\uis}{\ensuremath{u_1^l}}
\newcommand{\uts}{\ensuremath{u_2^l}}
\newcommand{\ups}{(\uis,\uts)}
\newcommand{\vis}{\ensuremath{v_1^k}}
\newcommand{\vts}{\ensuremath{v_2^k}}
\newcommand{\vps}{(\vis,\vts)}
\newcommand{\lpi}{_{\l+1}}
\renewcommand{\v}{u^{l-1}}
\newcommand{\w}{u^{l}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\CP}{\mbox{${\cal P}$}}
\renewcommand{\Pi}{\mathcal{P}}
%\renewcommand{\Theta}{\mathcal{D}}


\newlength{\lpskip}
\lpskip 4pt

\newcommand{\finv}{f_j^{-i}}
\newcommand{\ginv}{g_j^{-i}}

\newcommand{\cost}{\mbox{\rm cost}}
\newcommand{\seg}{\mbox{\rm seg}}
\newcommand{\segs}{\mbox{\rm segments}}
\newcommand{\valuex}{\mbox{\rm value}}
\newcommand{\rate}{\mbox{\rm rate}}
\newcommand{\spent}{\mbox{\rm spent}}
\newcommand{\all}{\mbox{\rm allocated}}
\newcommand{\allocated}{\mbox{\rm allocated}}
\newcommand{\ret}{\mbox{\rm returned}}
\newcommand{\good}{\mbox{\rm good}}
\newcommand{\best}{\mbox{\rm best}}
\newcommand{\bestT}{\mbox{\rm bestT}}
\newcommand{\fr}{\mbox{\rm fr}}
\newcommand{\fl}{\mbox{\rm fl}}
\newcommand{\bfr}{\mbox{\rm {\bf freeze}}}
\newcommand{\bpb}{\mbox{\rm bpb}}

\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\tS}{\ensuremath{\tilde{S}}}


%project specific
\newcommand{\alfail}{ \alpha_{il}}
\newcommand{\micap}{\hat{m}_i}
\newcommand{\sjcap}{\hat{s}_j}
\newcommand{\xijl}{ x_{ij}^l}
\newcommand{\uil}{ \u_{i}^l}
\newcommand{\lil}{ \lambda_{i}^l}
\newcommand{\muil}{ \mu_{i}^l}
\newcommand{\wil}{ w_{i}^l}
\newcommand{\bij}{ b_{ij}}
\newcommand{\bijl}{ b_{ij}^l}
\newcommand{\fij}{ f_{ij}}
\newcommand{\phij}{ \phi_{ij}}
\newcommand{\sca}{S \subseteq A}
\newcommand{\tcb}{T \subseteq B}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\poly}{\mathcal{P}}
\newcommand{\Lg}{{\mathcal{L}}_{\p}}
\newcommand{\one}{\mathds{1}}



\newcommand{\ipdf}[3]{
\begin{figure}[ht]
\label{#3}
\includegraphics[scale=#1]{#2}
\end{figure}
}










